PTPerf: On the performance evaluation of Tor Pluggable Transports

Tor, one of the most popular censorship circumvention systems, faces regular blocking attempts by censors. Thus, to facilitate access, it relies on "pluggable transports" (PTs) that disguise Tor's traffic and make it hard for the adversary to block Tor. However, these are not yet well studied and compared for the performance they provide to the users. Thus, we conduct a first comparative performance evaluation of a total of 12 PTs -- the ones currently supported by the Tor project and those that can be integrated in the future. Our results reveal multiple facets of the PT ecosystem. (1) PTs' download time significantly varies even under similar network conditions. (2) All PTs are not equally reliable. Thus, clients who regularly suffer censorship may falsely believe that such PTs are blocked. (3) PT performance depends on the underlying communication primitive. (4) PTs performance significantly depends on the website access method (browser or command-line). Surprisingly, for some PTs, website access time was even less than vanilla Tor. Based on our findings from more than 1.25M measurements, we provide recommendations about selecting PTs and believe that our study can facilitate access for users who face censorship.

==> Sections/Rough.tex <==
************Interpretation of paired t-test***************

Paired t-test (population p1, population p2)

If p<0.05
   Two populations are significantly different i.e., mean(P1) != mean(p2)
else
   Two populations are similar (rather we cannot say it's dissimilar)

For populations that are similar (i.e., p>0.05)
    and CI values(x,y) then x<0<y
Else
    0 must not be in the range (x,y)


**************************************

Commented first para of 4.2 Website access time

Commented first para of Conclusion

Last para of snowflake

==> Sections/body.tex <==








==> Sections/comparison.tex <==
\section{Pluggable Transports at a glance (a comparative analysis)}
\label{comparison}

\begin{table*}
\tiny
\centering
\begin{tabular}{|p{2.0cm}|p{1.0cm}|p{1.0cm}|p{1.1cm}|p{1.2 cm}|p{3.0cm}|p{2.2cm}|}
 \hline
 \multicolumn{7}{|c|}{\textbf{PTs bundled in the Tor Browser}} \\
 \hline
 \textbf{Name} &   \textbf{Code Available} &   \textbf{Functional} &   \textbf{Integratable} &   \textbf{Performance Evaluated} &   \textbf{Implementation challenges} &  \textbf{ Underlying technology}\\
 \hline
  Obfs4 \cite{obfs4} & \cmark & \cmark & \cmark & \cmark  &   None &   Random obfuscation \\
 \hline
 Meek \cite{meek} &  \cmark & \cmark & \cmark & \cmark  &   Requires CDN with domain fronting support &   Domain fronting \\
 \hline
  Snowflake \cite{snowflake} & \cmark & \cmark & \cmark & \cmark  &   Dependency on domain fronting &  WebRTC \\
 \hline
 
 \multicolumn{7}{|c|}{\textbf{PTs listed by the Tor project and currently under deployment/testing}} \\
 \hline
%  Name & Code-Availability & Functional & Integratable & Performance Evaluated? & PT server control & Implementation challenges & Underlying technology\\

  Dnstt \cite{dnstt} & \cmark & \cmark & \cmark & \cmark &   None &   DoH/DoT tunneling  \\
 \hline
  Conjure \cite{torConjure}  & \cmark & \cmark & \cmark & \cmark %\textdagger%
  &   Needs ISP support &   Decoy routing \\
 \hline
WebTunnel \cite{webTunnel} & \cmark & \cmark & \cmark & \cmark &   None &   Tunelling over HTTP  \\
 \hline
TorCloak \cite{torCloakmail, torCloakpdf} & \xmark & N/A & N/A & N/A & N/A &   Tunneling over WebRTC \\
 \hline
 
 \multicolumn{7}{|c|}{\textbf{PTs listed by the Tor project but undeployed}} \\
 \hline
 % Name & Code-Availability & Functional & Integratable & Performance Evaluated? & Ease of Customizability & Implementation challenges & Underlying technology\\

 Marionette \cite{dyer2015marionette} & \cmark & \cmark & \cmark & \cmark  &   Dependency issues (supports only Python 2.7) &   Network traffic obfuscation \\
 \hline
 Shadowsocks \cite{shadowsocks} & \cmark & \cmark & \cmark & \cmark  &   None &   Network traffic obfuscation \\
 \hline
 Stegotorus \cite{weinberg2012stegotorus} & \cmark & \cmark & \cmark & \cmark  &   None &   Steganographic obfuscation\\
 \hline
  Psiphon \cite{psiphon} & \cmark & \cmark & \cmark & \cmark  &   None &   Proxy-based\\
 \hline
% Dust \cite{wiley2011dust}& \cmark & \xmark & \xmark & N/A &   Missing ready to deploy code  &\\
 %\hline
 Lantern Lampshade \cite{lanternlampshade} & \cmark & \xmark & \xmark & N/A &   Unavailability of ready to deploy code  &   Obfuscated encryption\\
 \hline
 %\zu{Basket2} & \xmark & \xmark & \xmark & N/A & N/A & N/A \\
 %\hline
 
 \multicolumn{7}{|c|}{\textbf{PTs neither listed nor deployed by the Tor Project}} \\
 \hline
  %Name & Code-Availability & Functional & Integratable & Performance Evaluated? & Ease of Customizability & Implementation challenges & Underlying technology \\

 Cloak \cite{cloak} & \cmark & \cmark & \cmark & \cmark &   None &   Network traffic obfuscation \\
 \hline
 Camoufler \cite{sharma2021camoufler} & \cmark & \cmark & \cmark & \cmark  &   Dependency on IM    accounts &   Tunneling over IM application\\
 \hline
 Massbrowser \cite{nasr2020massbrowser} & \cmark & \cmark & \cmark & \cmark(partial)  &   Requires invite-code from authors &   domain fronting and browser based proxy \\
 \hline
 Protozoa \cite{protozoa} & \cmark & \xmark & \xmark & \xmark &   Code compilation issues &   Tunneling over WebRTC \\
 \hline
 Stegozoa \cite{figueira2022stegozoa} & \cmark & \xmark & \xmark & \xmark & Provides basic functionality, sends only text data over sockets &   Tunneling over WebRTC \\
 \hline
 Sweet \cite{zhou2012sweet} & \cmark & \xmark & \xmark & N/A &   Dependency issues &   Tunneling over emails)\\
 \hline
 Deltashaper \cite{barradas2017deltashaper} & \cmark & \xmark & \xmark & N/A &   Requires Skype version that is no longer supported &   Tunneling over video\\
 \hline
 Rook \cite{vines2015rook} & \cmark & \cmark & \xmark & N/A &   Can only be used for messaging; no proxy support &   Hiding data using online gaming \\
 \hline
 Facet \cite{facet} & \cmark & \xmark & \xmark & N/A &   Requires Skype version no that is longer supported  &   Tunneling over video \\
 \hline
 Mailet \cite{mailet} & \cmark & \cmark & \xmark & N/A &   Can only be used to access Twitter; no proxy support  &   Tunelling over email \\
 \hline
 MinecruftPT \cite{minecruft} & \cmark & \xmark & \xmark & N/A &  Issues in the source code\cite{issueMine} &   Hiding data using online gaming \\
 \hline
  %Httpt \cite{frolov2020httpt} & \cmark & \xmark & \xmark & N/A &   Source code not up to date &   Tunelling over HTTP \\\hline
 CloudTransport \cite{brubaker2014cloudtransport} & \xmark & N/A & N/A & N/A & N/A &   Tunneling over cloud\\
 \hline
 CovertCast \cite{mcpherson2016covertcast} & \xmark & N/A & N/A & N/A  & N/A &   Tunneling over video\\
 \hline
 FreeWave \cite{houmansadr2013want} & \xmark & N/A & N/A & N/A & N/A &   Tunneling over VoIP \\
 \hline
 Balboa \cite{rosen2021balboa} & \xmark & N/A & N/A & N/A & N/A &   Obfuscation based on user-traffic model\\
 \hline
 Domain Shadowing \cite{wei2021domain} & \xmark & N/A & N/A & N/A & N/A &   Domain-shadowing \\
 \hline
\end{tabular}

\caption{Comparison of Pluggable Transports}
\label{table:allpt}
\vspace{-3mm}
\end{table*}


In \Cref{sec:background}, we provided a brief description of different PTs that were evaluated in our study. However, 
the regular attempts to block Tor by China \cite{dunna2018analyzing}, coupled with the recent events of excessive banning of Tor and PTs by different regimes \cite{IR-block-Tor, Russia-ban-net3}, highlights the pressing need for more feasible options for PTs. Thus, in this work, we studied a total of 28 systems that could become PTs. But, many PTs were not part of our experiments for various reasons. With the help of Table~\ref{table:allpt}, we provide an overview of all the 28 PTs and the challenges involved in their adoption. 

The parameters in the table are suitably chosen for comparison. For instance, in the first row, for obfs4, we mention that its code was available, it is functional and integrated into Tor, and thus we measured its performance.
But for TorCloak the code is not publicly available, and thus we can not test it to ascertain whether it can be integrated with Tor. Thus we mark not applicable (\texttt{N/A}) in the respective fields.
Additionally, we could only partially test the working of the massbrowser. This is because it requires an access code to function for each unique device. We obtained only one access code from the authors, and thus we could test it from a single vantage point. For a fair comparison, we do not include it in our analysis, as we tested other PTs from several geographic locations.

Moreover, depending upon their adoption status by the Tor project, 
we categorize these PTs into broadly four categories---(1) PTs bundled with the Tor browser, (2) PTs listed by the Tor project and are under deployment and testing, (3) PTs listed by the Tor project and are not under deployment (4) PTs not listed by Tor.
Currently, only three PTs (obfs4, meek, and snowflake) are integrated with the Tor browser and can be easily used by the clients. 
Four are under deployment testing (\ie dnstt, conjure, webtunnel, and torcloak). The remaining 21 PTs are not under consideration for adoption. 
As previously stated, our goal was to deploy and run all these systems for performance comparisons. 
However, we found that 13 of the considered PTs were non-functional. We found multiple issues with them \eg source code not available, compilation errors, and deprecated versions of the underlying technology (mentioned in the table). Our analysis reveals that more focus should be given to the reproducibility of the proposed systems. 
Thus we plan to make our code and analysis scripts public to foster future research on PTs.
%We hope that our study may help the Tor community to further strengthen the PT ecosystem. \textbf{again repetitive}





% Following the recent events of excessive banning of Tor and PTs by different regimes, it becomes important to study what more technologies can be used as PTs. Thus, in \Cref{table:allpt}, we categorized the PTs such that it becomes easy to see what are the different challenges associated with PTs, what technology they use \etc












==> Sections/ethics.tex <==
\section{Ethical Considerations}
\label{sec:ethics}
In this research, we conducted a large-scale measurement campaign involving the live Tor network and Tor-supported pluggable transport infrastructure. Tor network is used by millions of users, and thus we ensured that our measurements should not impede regular Tor users. Thus we followed the principles prescribed in the Belmont report~\cite{beauchamp2008belmont}. The three important principles are:
\begin{itemize}
    \item Respect for persons: We did not involve any human subjects in our studies and thus did not require obtaining consent.
    \item Beneficence: In our study, we evaluate the performance of PTs over Tor which can ultimately result in enhanced user experience offering benefits to the users of the system.
    \item Justice: No user apart from the authors was involved in the experiments, and thus this study does not pose any risk to any third-party users. On the contrary, the outcomes of our research can benefit users for whom censorship is a daily reality.  
\end{itemize}

Since our experiments involved sending traffic over Tor, we carefully planned our measurements (spread out across multiple weeks) to not overload the Tor infrastructure. We conducted our experiments from VPSes hosted on cloud infrastructure at different locations and did not involve any residential networks.
We use standard Tor client utility similar to any regular Tor user. Throughout our experiments, we only accessed Tranco top-1k websites and CBL-1k, and file sizes of no more than 100 MB (hosted on our servers only). We took extra caution while performing our experiments involving pluggable transports that are used \textit{en masse} \eg Instant Messaging apps (camoufler), DNS resolvers (dnstt) \etc We ensured that at any point in time, we do not burden these systems (by running experiments in small batches).

For some experiments, we hosted our own Tor guard nodes on cloud-hosting machines. We used them only for accessing websites and downloading file sizes necessary for experiments. We never recorded any personally identifiable information of users (\eg IP address) connecting our guard nodes. Moreover, we hosted them only for the duration of the experiment. Across all our experiments we hosted a guard node maximum for a duration of four weeks after it received the guard status.
